Reverse Transition Kernel: A Flexible Framework to Accelerate Diffusion Inference

To generate data from trained diffusion models, most inference algorithms, such as DDPM, DDIM, and other variants, rely on discretizing the reverse SDEs or their equivalent ODEs. In this paper, we view such approaches as decomposing the entire denoising diffusion process into several segments, each corresponding to a reverse transition kernel (RTK) sampling subproblem. Specifically, DDPM uses a Gaussian approximation for the RTK, resulting in low per-subproblem complexity but requiring a large number of segments (i.e., subproblems), which is conjectured to be inefficient. To address this, we develop a general RTK framework that enables a more balanced subproblem decomposition, resulting in $\tilde O(1)$ subproblems, each with strongly log-concave targets. We then propose leveraging two fast sampling algorithms, the Metropolis-Adjusted Langevin Algorithm (MALA) and Underdamped Langevin Dynamics (ULD), for solving these strongly log-concave subproblems. This gives rise to the RTK-MALA and RTK-ULD algorithms for diffusion inference. In theory, we further develop the convergence guarantees for RTK-MALA and RTK-ULD in total variation (TV) distance: RTK-ULD can achieve $\epsilon$ target error within $\tilde{\mathcal O}(d^{1/2}\epsilon^{-1})$ under mild conditions, and RTK-MALA enjoys a $\mathcal{O}(d^{2}\log(d/\epsilon))$ convergence rate under slightly stricter conditions. These theoretical results surpass the state-of-the-art convergence rates for diffusion inference and are well supported by numerical experiments.

==> 0_config/init_load_icml_ver.tex <==
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{lipsum}         % Can be removed after putting your text content
\usepackage{natbib}
\usepackage{doi}
\usepackage{amssymb}
\usepackage{xcolor}         % colors
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{xspace}
\usepackage{lmodern}

\usepackage{enumitem}


% For paper revision:

\newcommand{\xh}[1]{\textcolor[HTML]{66CCFF}{#1}}
\def \dz {\textcolor{red}}

==> 0_config/math_commands_icml_ver.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


\newcommand{\issue}[1]{{\textcolor{purple}{#1} }}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvzeta{{\mathbf{\zeta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\cR{{\mathcal{R}}}
\def\EE{{\mathbb{E}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vrho{{\bm{\rho}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}




% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

%

\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny{#1}};}}
% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}[2]{\mathrm{KL}\left(#1 \big\| #2\right)}
\newcommand{\FI}[2]{\mathrm{FI}\left(#1 \| #2\right)}
\newcommand{\TVD}[2]{\mathrm{TV}\left(#1, #2\right)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\newcommand{\der}{\mathrm{d}}
\newcommand{\fder}{\mathrm{D}}
\newcommand{\rgrad}{\mathrm{grad}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Table settings

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}

% Lemma settings


%Specific Notations for Sampling along the Reverse Process with Recursive Score Estimation

\newcommand{\rbkwx}{\rvx^{\gets}}
\newcommand{\bkwx}{\vx^{\gets}}
\newcommand{\rbkwv}{\rvv^{\gets}}
\newcommand{\bkwv}{\vv^{\gets}}
\newcommand{\bkwp}{p^{\gets}}
\newcommand{\bkw}[1]{#1^{\gets}}

==> 0_contents/02preli_icml_ver.tex <==
\section{Preliminaries}
\label{sec:pre}

In this section, we first introduce the notations used in subsequent sections. 
Then, we present several distinct Markov processes to demonstrate the procedures for adding noise to existing data and generating new data. 
Besides, we specify the assumptions required for the target distribution in our algorithms and analysis.

\paragraph{Notations.}
We say a complexity $h\colon \R\rightarrow\R$ to be  $h(n)=\mathcal{O}(n^k)$ or $h(n)=\tilde{\mathcal{O}}(n^k)$ if the complexity satisfies $h(n)\le c\cdot n^{k}$ or $h(n)\le c\cdot n^{k}[\log (n)]^{k^\prime}$ for absolute contant $c, k$ and $k^\prime$.
We use the lowercase bold symbol $\rvx$ to denote a random vector, and the lowercase italicized bold symbol $\vx$ represents a fixed vector. 
The standard Euclidean norm is denoted by $\|\cdot\|$.
The data distribution is presented as $p_*\propto\exp(-f_*)$.
Besides, we define two Markov processes $\R^d$, i.e.,
\begin{equation*}
    \left\{\rvx_t\right\}_{t\in[0,T]},\quad  \left\{\rbkwx_{k\eta}\right\}_{k\in\{0,1,\ldots, K\}},\quad \mathrm{where}\quad T=K\eta.
\end{equation*}
In the above notations, $T$ presents the mixing time required for the data distribution to converge to specific priors, $K$ denotes the iteration number of the generation process, and $\eta$ signifies the corresponding step size. 
Further details of the two processes are provided below.

\paragraph{Adding noise to data with the forward process.}
The first Markov process $\{\rvx_t\}$ corresponds to generating progressively noised data from $p_*$.
In most denoising diffusion models, $\{\rvx_t\}$ is an Ornstein–Uhlenbeck (OU) process shown as follows
\begin{equation}
    \small
    \label{sde:ou}
    \der \rvx_t = -\rvx_t \der t + \sqrt{2}\der \mB_t \quad \mathrm{where}\quad \rvx_0\sim p_*\propto \exp(-f_*).
\end{equation}
If we denote underlying distribution of $\rvx_t$ as $p_t\propto \exp(-f_t)$ meaning $f_0 = f_*$,
the forward OU process provides an analytic form of the transition kernel, i.e.,
\begin{equation}
    \small
    \label{def:forward_trans_ker}
    \begin{aligned}
        p_{t^\prime|t}(\vx^\prime|\vx) = \frac{p_{t^\prime, t}(\vx^\prime, \vx)}{p_t(\vx)}\propto \exp \left[\frac{-\left\|\vx^\prime -e^{-(t^\prime-t)}\vx \right\|^2}{2\left(1-e^{-2(t^\prime-t)}\right)}\right]
    \end{aligned}
\end{equation}
for any $t^\prime\ge t$, where $p_{t^\prime,t}$ denotes the joint distribution of $(\rvx_{t^\prime}, \rvx_t)$.
According to the Fokker-Planck equation, we know the stationary distribution for SDE.~\eqref{sde:ou} is the standard Gaussian distribution.

\paragraph{Denoising generation with a reverse SDE.}
Various theoretical works~\citep{lee2022convergence,li2023towards,chen2022sampling, chen2023improved, benton2024nearly} based on DDPM~\citep{ho2020denoising} consider the generation process of diffusion models as the reverse process of SDE.~\eqref{sde:ou} denoted as $\{\rbkwx_t\}$.
According to the Doob’s $h$-Transform, the reverse SDE, i.e., $\{\rbkwx_t\}$, follows from
\begin{equation}
    \small
    \label{def:rev_ou_sde}
    \der \rbkwx_t = \left(\rbkwx_t + 2\grad\ln p_{T-t}(\rbkwx_t)\right)\der t + \sqrt{2}\der\mB_t,
\end{equation}
whose underlying distribution $p^\gets_{t}$ satisfies $p_{T-t} = p^\gets_{t}$.
Similar to the definition of transition kernel shown in Eq.~\ref{def:forward_trans_ker}, we define $p^\gets_{t^\prime|t}(\vx^\prime|\vx) = p^\gets_{t^\prime, t}(\vx^\prime,\vx)/p^\gets_t(\vx)$ for any $t^\prime\ge t\ge 0$ and name it as reverse transition kernel (RTK).

%In other words, if we denote the underlying distribution of $\rbkwx_t$ to be $\bkwp_t$, then we have $p_t = \bkwp_{T-t}$.
To implement SDE.~\eqref{def:rev_ou_sde}, diffusion models approximate the score function $\grad\ln p_{t}$ with a parameterized neural network model,  denoted by $\vs_{\vtheta,t}$, where $\vtheta$ denotes the network parameters.
% where $\vs_{\theta,T-t}$ can be obtained by minimizing the following objective function
% \begin{equation}
%     \label{def:dif_train_ori}
%     \min_{\theta}\ \E_{\rvx\sim p_t}\left[\left\|\grad \ln p_{t}(\rvx) - s_{\theta,t}(\rvx)\right\|^2\right]
% \end{equation}
% for any $0\le t\le T$.
% Although $\grad\ln p_t$ is unknown, this objective can be further reformulated as 
% \begin{equation}
%     \label{def:dif_train_prob}
%     \min_{\theta}\ \E\left[\left\|\vs_{\theta, t}(\rvx_t) + \frac{\xi_t}{\sqrt{1-e^{-2t}}}\right\|^2\right]
% \end{equation}
% due to the integration by parts technique shown in Appendix A of~\cite{chen2022sampling}.
% Note that the objective loss, i.e., Eq.~\eqref{def:dif_train_prob}, can be approximated by an empirical mean since $\rvx_t$ can be generated by the forward SDE.~\eqref{sde:ou}, i.e., $\rvx_t = e^{-t}\rvx_0 + \sqrt{1-e^{-2t}}\xi_t$ where $\xi_t\sim \mathcal{N}(\vzero,\mI)$ is independent of $\rvx_0$. 
Then, SDE.~\eqref{def:rev_ou_sde} can be implemented by
\begin{equation}
    \small
    \label{def:rev_ou_sde_prac}
    \der \overline{\rvx}_t = \left(\overline{\rvx}_t + 2 \vs_{\theta, T-k\eta}(\overline{\rvx}_{k\eta})\right)\der t + \sqrt{2}\der\mB_t
\end{equation}
for any $t\in[k\eta, (k+1)\eta)$ with a standard Gaussian initialization, $\overline{\rvx}_0 \sim \mathcal{N}(\vzero,\mI)$.
 Eq.~\eqref{def:rev_ou_sde_prac} has the following closed solution
\begin{equation}
    \small
    \label{def:rev_ou_sde_prac_closed}
    \overline{\rvx}_{(k+1)\eta} = e^{\eta}\cdot \overline{\rvx}_{k\eta} - 2(1-e^{\eta})\vs_{\theta, T-k\eta}(\overline{\rvx}_{k\eta}) + \sqrt{e^{2\eta}-1}\cdot\xi
\end{equation}
where $\xi\sim\mathcal{N}(\vzero,\mI)$.
This is exactly the DDPM algorithm.

\paragraph{DDPM approximately samples the reverse transition kernel.}
 DDPM can also be viewed as an approximated sampler for RTK, i.e., $p^\gets_{t^\prime|t}(\vx^\prime|\vx)$ for some $t'>t$. In particular, the update of DDPM at the iteration $k$ applies the Gaussian process $\overline{p}_{(k+1)\eta|k\eta}(\cdot|\vx)$ defined as
\begin{equation}
    \label{def:ddpm_trans_ker}
    \mathcal{N}\left(e^{\eta}\vx - 2(1-e^{\eta})\vs_{\theta,T-k\eta}(\vx), (e^{2\eta}-1)\cdot\mI\right)
\end{equation}
to approximate the distribution $p^\gets_{(k+1)\eta|k\eta}(\cdot|\vx)$ \citep{ho2020denoising}. Specifically, by the chain rule of KL divergence, the gap between the data distribution $p_*$ and the generated distribution  $\overline{p}_T$ satisfies
\begin{equation}\label{eq:chainrule_KL}
    \small
    \begin{aligned}
        &\KL{\overline{p}_T}{p_*} \le \KL{\overline{\rvx}_0}{p^\gets_0}\\
        &\quad + \sum_{k=0}^{K-1} \E_{\overline{\rvx}\sim \overline{p}_{k\eta}}\left[\KL{\overline{p}_{(k+1)\eta|k\eta}(\cdot|\overline{\rvx})}{p^\gets_{(k+1)\eta|k\eta}(\cdot|\overline{\rvx})}\right],
    \end{aligned}
\end{equation}
where $K = T/\eta$ is the total number of iterations. For DDPM, to guarantee a  small sampling error, we need to use a small step size $\eta$ to ensure that $\overline{p}_{(k+1)\eta|k\eta}$ is sufficiently close to $p^\gets_{(k+1)\eta|k\eta}$. Then, the required iteration numbers $K=T/\eta$ will be large and dominate the computational complexity. In \citet{chen2022sampling,chen2022improved}, it was shown that one needs to set $\eta = \tilde{\mathcal{O}}(\epsilon^2)$ to achieve $\epsilon$ sampling error in TV distance (assuming no score estimation error) and the total complexity is $K=\tilde{\mathcal{O}}(1/\epsilon^2)$.

% Although implementing DDPM-based methods with Eq.~\eqref{def:rev_ou_sde_prac} is intuitive and practical, like discretizing SDE for the continuous Langevin dynamics, it is also biased and inefficient.


% Specifically, the KL divergence gap between the underlying distribution of $\tilde{\rvx}_T$ (generated data) and $\rvx_0$ (real data) satisfies
% \begin{equation*}
%     \small
%     \KL{\overline{p}_T}{p_0} \le \KL{\overline{\rvx}_0}{p_T} + \sum_{k=0}^{K-1} \E_{\overline{\rvx}\sim \overline{p}_{k\eta}}\left[\KL{\overline{p}_{(k+1)\eta|k\eta}(\cdot|\overline{\rvx})}{p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\overline{\rvx})}\right].
% \end{equation*}
% This inequality indicates that if we consider the generation process as a posterior sampling problem, it can be implemented by solving a series of sampling subproblems whose target distribution is the reverse transition kernel (RTK) of the forward process, i.e., $p_{(K-k-1)\eta|(K-k)\eta}$.
% DDPM utilizes Eq.~\eqref{def:rev_ou_sde_prac} to update particles, which is equivalent to set 
% \begin{equation}
%     \label{def:ddpm_trans_ker}
%     \overline{p}_{(k+1)\eta|k\eta}(\cdot|\vx)  = \mathcal{N}\left(e^{\eta}\vx - 2(1-e^{\eta})\vs_{\theta,T-k\eta}(\vx), (e^{2\eta}-1)\cdot\mI\right).
% \end{equation}
% Although such Gaussian-type distributions can be implemented efficiently, the iteration number $ K=T/\eta$ required in the generation process will be large and dominate the computational complexity.
% This is because the Girsanov theorem~\citep{sarkka2019applied} shows that the gap between the ideal transition kernel $p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\overline{\rvx})$ and the practical one $\overline{p}_{(k+1)\eta|k\eta}(\cdot|\overline{\rvx})$ can be upper bounded by the integration of the drift term gaps, i.e.,
% \begin{equation}
%     \begin{aligned}
%         \label{ineq:kl_gap_girsanov}
%     &\E_{\overline{\rvx}\sim \overline{p}_{k\eta}}\left[\KL{\overline{p}_{(k+1)\eta|k\eta}(\cdot|\overline{\rvx})}{p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\overline{\rvx})}\right]\\
%     &= \int_{0}^{\eta}\E\left[\left\|\vs_{\theta, T-k\eta}(\overline{\rvx}_{k\eta}) - \grad\ln p_{T-(k\eta+\tau)}(\overline{\rvx}_{k\eta+\tau})\right\|^2\right]\der \tau.
%     \end{aligned}
% \end{equation}
% Even if we omit the approximation error between $\vs_{\theta, T-k\eta}$ and $\grad\ln p_{T-k\eta}$, we need to set $\eta = \tilde{\mathcal{O}}(\epsilon^2)$ to keep Eq.~\eqref{ineq:kl_gap_girsanov} and the final KL divergence gap sufficiently small, i.e., $\KL{\overline{p}_T}{p_0}\le \epsilon$~\citep{chen2022sampling,chen2023improved}, which means the iteration number should satisfy $K=\tilde{\mathcal{O}}(\epsilon^{-2})$.

\paragraph{Intuition for General Reverse Transition Kernel.}
As previously mentioned, DDPM approximately solves RTK sampling subproblems using a small step size $\eta$. While this allows for efficient one-step implementation, it necessitates a large number of RTK sampling problems. This naturally creates a trade-off between the quantity of RTK sampling problems and the complexity of solving them. To address this, one can consider a larger step size $\eta$, which results in a relatively more challenging RTK sampling target $p^\gets_{(k+1)\eta|k\eta}$ and a reduced number of sampling problems ($K=T/\eta$). By examining a general choice for the step size $\eta$, the generation process of diffusion models can be depicted through a comprehensive framework of reverse transition kernels, which will be explored in depth in the following section. This framework enables the design of various decompositions for RTK sampling problems and algorithms to solve them, resulting in an extensive family of generation algorithms for diffusion models (that encompasses DDPM). Consequently, this also offers the potential to develop faster algorithms with lower computational complexities, e.g., applying fast sampling algorithms for sampling the RTK, i.e., $p^\gets_{(k+1)\eta|k\eta}$ with a properly large $\eta$.


\paragraph{General Assumptions.} Similar to the analysis of DDPM~\citep{chen2022sampling,chen2023improved}, we make the following  assumptions on the data distribution $p_*$ that will be utilized in the theory.

\begin{enumerate}[label=\textbf{[A{\arabic*}]}]
    \item \label{ass:lips_score} For all $t\ge 0$, the score $\grad \ln p_{t}$ is $L$-Lipschitz.
    \item \label{ass:second_moment} The second moment of the target distribution $p_*$ is upper bounded, i.e., $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2}\right]=m_2^2$.
    % \item \label{ass:score_approximation} For all $k=0, 1,\ldots, K$, it has
    % \begin{equation*}
    %     \E_{\rvx\sim p_{k\eta}}\left[\left\|s_{\theta}(\rvx, k\eta) - \grad \log p_{k\eta}(\rvx)\right\|^2\right]\le \epsilon^2_{\mathrm{score}}.
    % \end{equation*}
\end{enumerate}
Assumption~\ref{ass:lips_score} is standard one in diffusion literature and has been used in many prior works~\citep{block2020generative, chen2022improved, lee2022convergence, chen2024probability}.
Moreover, we do not require the isoperimetric conditions, e.g., the establishment of the log-Sobolev inequality and the Poincar\'e inequality for the data distribution $p_*$ as~\cite{lee2022convergence}, and the convex conditions for the energy function $f_*$ as~\cite{block2020generative}.
Therefore, our assumptions cover a wide range of highly non-log-concave data distributions.
We emphasize that Assumption~\ref{ass:lips_score} may be relaxed only to assume the target distribution is smooth rather than the entire OU process, based on the technique in \cite{chen2023improved} (see rough calculations in their Lemmas 12 and 14).
We do not include this additional relaxation in this paper to clarify our analysis.
Assumption~\ref{ass:second_moment} is one of the weakest assumptions being adopted for the analysis of posterior sampling.
% In this work, we construct a novel Markov process that approximates the forward RTK with strongly log-concave distributions rather than a Gaussian-type distribution as shown in Eq.~\eqref{def:ddpm_trans_ker}.
% Considering that strongly log-concave distributions are more general than the Gaussian-type distributions, it potentially has the ability to approximate $p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\tilde{\rvx})$ with a larger $\eta$, and then decrease the iteration number $K$ required in the generation process.
% On the other hand, acceleration techniques used to draw samples from strongly log-concave distributions have been well-explored in posterior sampling tasks. 
% We expect the complexity for solving the sampling subproblem will exhibit only a limited growth compared with sampling from the Gaussian, i.e., Eq.~\eqref{def:ddpm_trans_ker}, directly.


==> 0_contents/03framework_icml_ver.tex <==
\section{General Framework of Reverse Transition Kernel}
\label{sec:framework}
This section introduces the general framework of Reverse Transition Kernel (RTK).
As mentioned in the previous section, the framework is built upon the general setup of segmentation: each segment has length $\eta$; within each segment, we generate samples according to the RTK target distributions. Then, the entire generation process in diffusion models can be considered as the combination of a series of sampling subproblems. In particular, the inference process via RTK is displayed in Alg. \ref{alg:rtk}. 

% Then, we introduce how to choose the target distribution of sampling subproblems to balance the number and difficulty of these subproblems.
% Finally, we provide sufficient conditions for closing the distribution gap between the output particles and the real data to an arbitrary accuracy.

\begin{algorithm}
    \caption{\sc Inference with Reverse Transition Kernel (RTK)}
    \label{alg:rtk}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} Initial particle $\hat{\rvx}_0$ sampled from the standard Gaussian distribution, Iteration number $K$, Step size $\eta$, required convergence accuracy $\epsilon$;
            \FOR{$k=0$ to $K-1$}
                \STATE \label{step:inner_sampler} Draw sample $\hat{\rvx}_{(k+1)\eta}$ with MCMCs from $\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta})$ which is closed to the ground-truth reverse transition kernel, i.e.,
                \begin{equation}
                    \small
                    \label{def:inner_target_dis}
                    \begin{aligned}
                        &p^\gets_{(k+1)\eta|k\eta}(\vz|\hat{\rvx}_{k\eta})\propto \exp\left(-g(\vz)\right)\\
                        & \coloneqq \exp\left( -f_{(K-k-1)\eta}(\vz)-\frac{\left\|\hat{\rvx}_{k\eta} - \vz\cdot e^{-\eta}\right\|^2}{2(1-e^{-2\eta})}\right).
                    \end{aligned}
                \end{equation}
                % with access only to the score approximations: $s_{\theta, T-(k+1)\eta}\approx \grad f_{T-(k+1)\eta}$. 
                %\textcolor{blue}{[You mean $\grad \ln p_{T-(k+1)\eta}$? I think you defined $p_*\propto \exp(-f_*)$.]}
                %\textcolor{blue}{Actually can we just say: sample from $\exp\left( s_{\theta,{(K-k-1)\eta}}(\hat{\rvx}_{(k+1)\eta})-\frac{\left\|\hat{\rvx}_{k\eta} - \hat{\rvx}_{(k+1)\eta}\cdot e^{-\eta}\right\|^2}{2(1-e^{-2\eta})}\right)$ with MALA or ULA (Algorithm 2 or 3)?}
            \ENDFOR
            \STATE {\bfseries return} $\hat{\rvx}_{K}$.
    \end{algorithmic}
\end{algorithm}

\paragraph{The implementation of RTK framework.}
We begin with a new Markov process $\{\hat{\rvx}_{k\eta}\}_{k=0,1,\ldots,K}$ satisfying $K\eta = T$, where the number of segments $K$, segment length $\eta$, and length of the entire process $T$ correspond to the definition in Section~\ref{sec:pre}.
Consider the Markov process $\{\hat{\rvx}_{k\eta}\}$ as the generation process of diffusion models with underlying distributions $\{\hat{p}_{k\eta}\}$, we require $\hat{p}_0 = \mathcal{N}(\vzero,\mI)$ and $\hat{p}_{K\eta}\approx p_*$, which is similar to the Markov process $\{\rbkwx_{k\eta}\}$.
In order to make the underlying distribution of output particles close to the data distribution, we can generate $\hat{\rvx}_{k\eta}$ with Alg.~\ref{alg:rtk}, which is equivalent to the following steps:
\begin{itemize}[leftmargin=*]
    \item Initialize $\hat{\rvx}_0$ with an easy-to-sample distribution, e.g., $\mathcal{N}(\vzero,\mI)$, which is closed to $p_{K\eta}$.
    \item Update particles by drawing samples from $\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta})$, which satisfies $$\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta})\approx p^\gets_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta}).$$ 
\end{itemize}
Under these conditions, if $\hat{p}_{k\eta}(\vz)\approx p_{(K-k)\eta}(\vz)$ , then we have
\begin{equation*}
    \begin{aligned}
        \hat{p}_{(k+1)\eta}(\vz) & = \left<\hat{p}_{(k+1)\eta|k\eta}(\vz|\cdot), \hat{p}_{k\eta}(\cdot)\right>\\
        & \approx \left<p^\gets_{(k+1)\eta|k\eta}(\vz|\cdot), p^\gets_{k\eta}(\cdot)\right> = p_{(k+1)\eta}(\vz)
    \end{aligned}
\end{equation*}
for any $k\in\{0,1,\ldots, K\}$.
This means we can implement the generation of diffusion models by solving a series of sampling subproblems with target distributions $p^\gets_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta})$.


\paragraph{The closed form of reverse transition kernels.\quad}
To implement Alg.~\ref{alg:rtk}, the most critical problem is determining the analytic form of RTK $p^\gets_{t^\prime|t}(\vx^\prime|\vx)$ for and $t^\prime\ge t\ge 0$ which is shown in the following lemma whose proof is deferred to Appendix~\ref{sec:appendix_rtk_framework}.
\begin{lemma}
    \label{lem:rev_trans_ker_form}
    Suppose a Markov process $\{\rvx_t\}$ with SDE.~\ref{sde:ou}, then for any $t^\prime > t$, we have
    \begin{equation*}
        \begin{aligned}
            &p^\gets_{T-t|T-t^\prime}(\vx|\vx^\prime) = p_{t|t^\prime}(\vx|\vx^\prime)\\
            &\propto \exp\left(-f_t(\vx)-\frac{\left\|\vx^\prime - \vx\cdot e^{-(t^\prime-t)}\right\|^2}{2(1-e^{-2(t^\prime-t)})}\right).
        \end{aligned}
    \end{equation*}
\end{lemma}
% Lemma~\ref{lem:rev_trans_ker_form} is proved in Appendix~\ref{sec:not_ass_app} by checking the establishment of the following equation, i.e.,
% \begin{equation*}
%     p_t(\vx) = \int p_{t|t^\prime}(\vx|\vx^\prime) p_{t^\prime}(\vx^\prime) \der\vx^\prime = \int p_{t|t^\prime}(\vx|\vx^\prime) \cdot\left[\int p_t(\vy) p_{t^\prime|t}(\vx^\prime|\vy) \der \vy\right]\der\vx^\prime,
% \end{equation*}
% which follows from Bayes' theorem.
% Note that in the above equation, the transition kernel, i.e., $p_{t^\prime|t}$, can be obtained explicitly as Eq.~\ref{def:forward_trans_ker} in the forward OU process.
The first critical property shown in this Lemma is that RTK $p_{t|t^\prime}$ is a perturbation of $p_t$ with a $l_2$ regularization.
This means if the score of $p_t$, i.e., $\grad f_t$, can be well-estimated, the score of RTK, i.e., $\grad \log p_{t|t^\prime}$ can also be approximated with high accuracy.
Moreover, in the diffusion model, $\grad f_t=\nabla \log p_t$ is exactly the score function at time $t$, which is approximated by the score network function $\vs_{\theta,t}(\vx)$, then
% since we are considering the generation process of denoising diffusion models, the training loss Eq.~\ref{def:dif_train_ori} is designed to provide a highly accurate score estimation for $p_t$.
\begin{equation*}
    \begin{aligned}
        & -\grad\log p_{t|t^\prime}(\vx|\vx^\prime) = \grad f_t(\vx) + \frac{e^{-2(t^\prime - t)}\vx - e^{-(t^\prime - t)}\vx^\prime}{1-e^{-2(t^\prime - t)}}\\
        & \approx \vs_{\theta, t}(\vx) + \frac{e^{-2(t^\prime - t)}\vx - e^{-(t^\prime - t)}\vx^\prime}{1-e^{-2(t^\prime - t)}},
    \end{aligned}
\end{equation*}
which can be directly calculated with a single query of $\vs_{\theta,t}(\vx)$.
The second critical property of RTK is that we can control the spectral information of its score by tuning the gap between $t^\prime$ and $t$.
Specifically, considering the target distribution, i.e., $p_{(K-k-1)\eta|(K-k)\eta}$ for the $k$-th transition, the Hessian matrix of its energy function satisfies
\begin{equation*}
    \begin{aligned}
        & - \grad^2 \log p_{(K-k-1)\eta|(K-k)\eta}\\
        & = \grad^2 f_{(K-k-1)\eta}(\vx) +  \frac{e^{-2\eta}}{1-e^{-2\eta}}\cdot \mI.
    \end{aligned}
\end{equation*}
According to Assumption~\ref{ass:lips_score}, the Hessian
\begin{equation*}
    \grad^2 f_{(K-k-1)\eta}(\vx)=-\grad^2 \log p_{(K-k-1)\eta}
\end{equation*}
can be lower bounded by $-L\mI$, which implies that RTK $p_{(K-k-1)\eta|(K-k)\eta}$ will be $L$-strongly log-concave and $3L$-smooth when the step size is set $\eta= 1/2\cdot \log (1+1/2L)$.
This further implies that the targets of all subsampling problems in Alg. \ref{alg:rtk} will be strongly log-concave, which can be sampled very efficiently by various posterior sampling algorithms.




\paragraph{Sufficient conditions for the convergence.\quad}
% To accurately describe the KL divergence gap between $\hat{p}_{K\eta}$ and $p_*$, we can introduce the chain rule of KL divergence of TV distance, e.g.,
% \begin{equation*}
%     \small
%     \KL{\hat{p}_{K\eta}}{p_*} \le \KL{\hat{p}_0}{p_T} + \sum_{k=0}^{K-1} \E_{\hat{\rvx}\sim \hat{p}_{k\eta}}\left[\KL{\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx})}{p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\hat{\rvx})}\right].
% \end{equation*}
% This means that high-quality generation requires proper initialization and accurate solutions for sampling subproblems. 
% Specifically, we have the following Lemma.
According to Pinsker's inequality and Eq. \eqref{eq:chainrule_KL}, the we can obtain the following lemma that establishes the general error decomposition for Alg.\ref{alg:rtk}.
\begin{lemma}
    \small
    \label{lem:num_diff_balance_kl}
    For Alg~\ref{alg:rtk}, we have
    \begin{align*}
        \TVD{\hat{p}_{K\eta}}{p_*}\le  \sqrt{(1+L^2)d + \left\|\grad f_*(\vzero)\right\|^2} \cdot \exp(-K\eta) \\
        + \sqrt{\frac{1}{2}\sum_{k=0}^{K-1} \E_{\hat{\rvx}\sim \hat{p}_{k\eta}}\left[\KL{\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx})}{\bkwp_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx})}\right]} 
    \end{align*}
    for any $K\in \mathbb{N}_+$ and $\eta\in\R_+$.
\end{lemma}
% Revisiting the chain rule of KL divergence with Lemma~\ref{lem:rev_trans_ker_form} and Lemma~\ref{lem:kl_inner_conv}, 
It is worth noting that the choice of $\eta$ represents a trade-off between the number of subproblems divided throughout the entire process and the difficulty of solving these subproblems. By considering the choice $\eta= 1/2\cdot \log (1+1/2L)$, we can observe two points: (1) the sampling subproblems in Alg.~\ref{alg:rtk} tend to be simple, as all RTK targets, presented in Lemma~\ref{lem:rev_trans_ker_form}, can be provably strongly log-concave; (2) the total number of subproblems is $K = T/\eta = \tilde{\mathcal O}(1)$, which is not large. Conversely, when considering a larger $\eta$ that satisfies $\eta\gg \log (1+1/L)$, the RTK target will no longer be guaranteed to be log-concave, resulting in high computational complexity, potentially even exponential in $d$, when solving the corresponding sampling subproblems. On the other hand, if a much smaller step size $\eta = o(1)$ is considered, the target distribution of the sampling subproblems can be easily solved, even with a one-step Gaussian process. However, this will increase the total number of sampling subproblems, potentially leading to higher computational complexity.

Therefore, we will consider the setup $\eta = 1/2\cdot \log(1+1/2L)$ in the remaining part of this paper. Now, the remaining task, which will be discussed in the next section, would be designing and analyzing the sampling algorithms for implementing all iterations of Alg.~\ref{alg:rtk}, i.e., solving the subproblems of RTK. 



% Besides, Lemma~\ref{lem:kl_inner_conv} requires the KL convergence to RTK for the sampling subproblems, which is a relatively strict condition for some posterior samplers, e.g., Metropolis-Adjusted Langevin Algorithm (MALA)~\citep{Roberts2014Langevin,Xifara2014Langevin}. 
% Therefore, we provide another Lemma that only requires the TV convergence to RTK for the sampling subproblems.

% \begin{lemma}
%     \label{lem:num_diff_balance_tv}
%     For Alg~\ref{alg:rtk}, we have
%     \begin{align*}
%         \TVD{\hat{p}_{K\eta}}{p_*}\le & \sqrt{(1+L^2)d + \left\|\grad f_*(\vzero)\right\|^2} \cdot \exp(-K\eta) \\ &+ \sum_{k=0}^{K-1} \E_{\hat{\rvx}\sim \hat{p}_{k\eta}}\left[\TVD{\hat{p}_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx})}{\bkwp_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx})}\right] 
%     \end{align*}
%     for any $K\in \mathbb{N}_+$ and $\eta\in\R_+$.
% \end{lemma}

\section{Implementation of RTK inner loops}

In this section, we outline the implementation of Step~\ref{step:inner_sampler} in the RTK algorithm, which aims to solve the sampling subproblems with strong log-concave targets, i.e., $p^\gets_{(k+1)\eta|k\eta}(\cdot|\hat{\rvx}_{k\eta})\propto \exp(-g)$.
Specifically, we employ two MCMC algorithms, i.e., the Metropolis-adjusted Langevin algorithm (MALA) and underdamped Langevin dynamics (ULD).
For each algorithm, we will first introduce the detailed implementation, combined with some explanation about notations and settings to describe the inner sampling process.
After that, we will provide general convergence results and discuss them in several theoretical or practical settings.
Besides, we will also compare our complexity results with the previous ones when achieving the convergence of TV distance to show that the RTK framework indeed obtains a better complexity by balancing the number and complexity of sampling subproblems.

\begin{algorithm}[t]
    \caption{\sc MALA/Projected MALA for RTK Inference}
    \label{alg:inner_mala}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:}  Returned particle of the previous iteration $\vx_0$, current iteration number $k$, inner iteration number $S$, inner step size $\tau$, required convergence accuracy $\epsilon$;
            \STATE Draw the initial particle $\rvz_0$ from 
            \begin{equation*}
                \frac{\mu_0(\der \vz)}{\der \vz} \propto \exp\left(-L\|\vz\|^2 - \frac{\left\|\vx_0 - e^{-\eta}\vz\right\|^2}{2(1-e^{-2\eta})}\right).
            \end{equation*}
            \FOR{$s=0$ to $S-1$}
                \STATE \label{step:ula} Draw a sample $\tilde{\vz}_s$ from the Gaussian distribution $\mathcal{N}(\vz_s - \tau\cdot s_{\theta}(\vz_s) ,2\tau\mI)$;
                \IF{$\vz_{s+1}\not\in\mathcal{B}(\vz_s, r)\cap\mathcal{B}(\vzero, R)$} \label{step:inball}
                    \STATE {$\vz_{s+1} = \vz_s$}; \COMMENT{This condition step is only activated for Projected MALA.}
                    \STATE \textbf{continue};
                \ENDIF
                \STATE Calculate the accept rate as
                \begin{equation*}
                    \small
                    \begin{aligned}
                        &a(\tilde{\vz}_s - (\vz_s-\tau\cdot s_\theta(\vz_s)), \vz_s)  \\ &=\min\left\{1, \exp\left(r(\vz_s,\tilde{\vz}_s) 
                        +  \frac{\left\|\tilde{\vz}_s - \vz_s +\tau\cdot s_\theta(\vz_s)\right\|^2 }{4\tau}\right.\right.\\
                        &\qquad \qquad\qquad \qquad \left.\left. -\frac{\left\|\vz_s-\tilde{\vz}_s+\tau\cdot s_\theta(\tilde{\vz}_s)\right\|^2}{4\tau}\right)\right\};
                    \end{aligned}
                \end{equation*}
                \STATE Update the particle $\vz_{s+1} = \tilde{\vz}_s$ with probability $a$, otherwise $\vz_{s+1}=\vz_s$.
            \ENDFOR
            \STATE {\bfseries return} $\rvz_{S}$;
    \end{algorithmic}
\end{algorithm}

\paragraph{RTK-MALA.\quad}
Alg.~\ref{alg:inner_mala} presents a solution employing MALA for the inner loop. When it is used to solve the $k$-th sampling subproblem of Alg.~\ref{alg:rtk}, $\vx_0$ is equal to $\hat{\rvx}_{k\eta}$ defined in Section~\ref{sec:framework} and used to initialize particles iterating in Alg.~\ref{alg:inner_mala}.
In Alg.~\ref{alg:inner_mala}, we consider the process $\{\rvz_s\}_{s=0}^S$ whose underlying distribution is denoted as $\{\mu_s\}_{s=0}^{S}$.
Although we expect $\mu_S$ to be close to the target distribution $p^\gets_{(k+1)\eta|k\eta}(\cdot|\vx_0)$, in real practice, the output particles $\rvz_S$ can only approximately follow $p^\gets_{(k+1)\eta|k\eta}(\cdot|\vx_0)$ due to inevitable errors.
Therefore, these errors should be explained in order to conduct a meaningful complexity analysis of the implementable algorithm.
Specifically, Alg.~\ref{alg:inner_mala} introduces two intrinsic errors:
\begin{enumerate}[label=\textbf{[E{\arabic*}]}]
    \item \label{e1}Estimation error of the score function: we assume a score estimator, e.g., a well-trained diffusion model, $s_{\theta}$, which can approximate the score function with an $\epsilon_{\mathrm{score}}$ error, i.e., $\left\|s_{\theta,t}(\vz) - \grad \log p_t(\vz)\right\|\leq \epsilon_{\mathrm{score}}$  for all $\vz\in\RR^d$ and $t\in[0,T]$.
    \item \label{e2}Estimation error of the energy function difference:  we assume an energy difference estimator $r$ which can approximate energy difference with an $\epsilon_{\mathrm{energy}}$ error, i.e.,
    $\left| r_t(\vz^\prime, \vz) + \log p_t(\vz^\prime) - \log p_t(\vz) \right|\leq \epsilon_{\mathrm{energy}}$ for all $\vz,\vz'\in\RR^d$.
\end{enumerate}

Under these settings, we provide a general convergence theorem for Alg.~\ref{alg:inner_mala}.
To clearly convey the convergence properties, we only show an informal version.
\begin{theorem}[Informal version of Theorem~\ref{thm:nn_estimate_complexity_gene}]
    \label{thm:nn_estimate_complexity_gene_informal}
    Under Assumption~\ref{ass:lips_score}--\ref{ass:second_moment}, for Alg.~\ref{alg:rtk}, we choose 
    \begin{equation*}
        \small
        \begin{aligned}
             \eta= \frac{1}{2}\log \frac{2L+1}{2L},\quad K = 4L\cdot \log \frac{(1+L^2)d+\left\|\grad f_*(\vzero)\right\|^2}{\epsilon^2}
        \end{aligned}
    \end{equation*}
    and implement Step 3 of Alg.~\ref{alg:rtk} with Alg.~\ref{alg:inner_mala}.
    Suppose the score~\ref{e1}, energy~\ref{e2} estimation errors and the inner step size $\tau$ satisfy
    \begin{equation*}
        \begin{aligned}
            &\epsilon_{\mathrm{score}} = \mathcal{O}(\rho d^{-1/2}),\quad  \epsilon_{\mathrm{energy}} = \mathcal{O}(\rho \tau^{1/2}),\\
            &\tau = \tilde{\mathcal{O}}\left(L^{-2}\cdot (d+m_2^2+Z^2)^{-1}\right),
        \end{aligned}
    \end{equation*}
    and the hyperparameters, i.e., $R$ and $r$, are chosen properly. 
    We have
    \begin{equation}
        \label{tv:con_rate}
        \small
        \begin{aligned}
            \TVD{\hat{p}_{K\eta}}{p_*}\le &\tilde{\mathcal{O}}(\epsilon) + \exp\left(\mathcal{O}(L(d+m_2^2))\right)\cdot \left(1- \frac{\rho^2}{4} \cdot \tau\right)^S\\
            &+ \tilde{\mathcal{O}}\left(\frac{Ld^{1/2}\epsilon_{\mathrm{score}}}{\rho}\right) + \tilde{\mathcal{O}}\left(\frac{L\epsilon_{\mathrm{energy}}}{\rho\tau^{1/2}}\right)
        \end{aligned}
    \end{equation}
    where $\rho$ is the Cheeger constant of a truncated inner target distribution $\exp(-g(\vz))\vone[\vz\in\mathcal{B}(\vzero,R)]$ and $Z$ denotes the maximal $l_2$ norm of particles appearing in Alg.~\ref{alg:rtk}.
\end{theorem}

It should be noted that the choice of $\eta$ choice ensures the $L$ strong log-concavity of target distribution $\exp(-g(\vz))$, which means its Cheeger constant is also $L$.
Although the Cheeger constant $\rho$ in the second term of Eq.~\ref{tv:con_rate} corresponding to truncated $\exp(-g(\vz))$ should also be near $L$ intuitively, current techniques can only provide a loose lower bound at an $\mathcal{O}(\sqrt{L/d})$-level (proven in Corollary~\ref{cor:cheeger_truncation}).
While in both cases above, the Cheeger constant is independent with $\epsilon$.
Combining this fact with an $\epsilon$-independent choice of inner step sizes $\tau$, the second term of Eq.~\ref{tv:con_rate} will converge linearly with respect to $\epsilon$.
As for the diameter $Z$ of particles used to upper bound $\tau$, though it may be unbounded in the standard implementation of Alg.~\ref{alg:inner_mala}, Lemma~\ref{lem:particles_z_bound} can upper bound it with $\tilde{\mathcal{O}}\left(L^{3/2}(d+m_2^2) \rho^{-1}\right)$ under the projected version of Alg.~\ref{alg:inner_mala}.

Additionally, to require the final sampling error to satisfy $\TVD{\hat{p}_{K\eta}}{p_*}\le \tilde{\mathcal{O}}(\epsilon)$, Eq.~\ref{tv:con_rate} shows that the score and energy difference estimation errors should be $\epsilon$-dependent and sufficiently small, where $\epsilon_{\mathrm{score}}$ corresponding to the training loss can be well-controlled.
However, obtaining a highly accurate energy difference estimation (requiring a small $\epsilon_{\mathrm{energy}}$) is hard with only diffusion models.
To solve this problem, we can introduce a neural network energy estimator similar to~\cite{xu2024provably} to construct $r(\vz^\prime, \vz,t)$, which induces the following complexity describing the calls of the score estimation.


\begin{corollary}[Informal version of Corollary~\ref{cor:complexity_19}]
    \label{cor:complexity_19_informal}
    Suppose the estimation errors of score and energy difference satisfy
    \begin{equation*}
        \epsilon_{\mathrm{score}}\le \frac{\rho\epsilon}{Ld^{1/2}}\quad \mathrm{and}\quad \epsilon_{\mathrm{energy}}\le \frac{\rho\epsilon}{L^2\cdot (d^{1/2}+m_2+Z)},
    \end{equation*}
    If we implement Alg.~\ref{alg:rtk} with the projected version of Alg.~\ref{alg:inner_mala} with the same hyperparameter settings as Theorem~\ref{thm:nn_estimate_complexity_gene_informal}, it has $\TVD{\hat{p}_{K\eta}}{p_*}\le \tilde{\mathcal{O}}(\epsilon)$
    with an $\mathcal{O}(L^4 \rho^{-2}\cdot \left(d+m_2^2\right)^2 Z^2\cdot \log (d/\epsilon) )$ complexity.
\end{corollary}

Considering the loose bound for both $\rho$ and $Z$, the complexity will be at most $\tilde{\mathcal{O}}(L^5(d+m_2^2)^6)$ which is the first linear convergence w.r.t. $\epsilon$ result for the diffusion inference process.

\paragraph{Score-only RTK-MALA.}
However, the parametric energy function may not always exist in real practice. We consider a more practical case where only the score estimation is accessible. In this case, we will make use of estimated score functions to approximate the energy difference, leading to the score-only RTK-MALA algorithm. In particular, recall that the energy difference function takes the following form:
\begin{equation*}
    \small
    \begin{aligned}
        g(\vz^\prime) - g(\vz) =  &-\log p_{(K-k-1)\eta}(\vz^\prime)+\frac{\left\|\vx_0 - \vz^\prime\cdot e^{-\eta}\right\|^2}{2(1-e^{-2\eta})}\\
        & +\log p_{(K-k-1)\eta}(\vz) - \frac{\left\|\vx_0 - \vz\cdot e^{-\eta}\right\|^2}{2(1-e^{-2\eta})}.
    \end{aligned}
\end{equation*}
Since the quadratic term can be obtained exactly, we only need to estimate the energy difference. Then let $f(\vz) = -\log p_{(K-k-1)\eta}(\vz)$ and denote $h(t) = f\left( \left(\vz^\prime - \vz\right)\cdot t + \vz\right)$, 
% $f_{(K-k-1)\eta}$ presented as $f$ for abbreviation. 
% With the following function
% \begin{equation*}
%     h(t) = f\left( \left(\vz^\prime - \vz\right)\cdot t + \vz\right),
% \end{equation*}
the energy difference $g(\vz^\prime) - g(\vz)$ can be reformulated as
\begin{equation*}
    h(1)-h(0) = \sum_{i=1} \frac{h^{(i)}(0)}{i!}\quad \mathrm{and}\quad h^{(i)}(t) \coloneqq \frac{\der^i h(t)}{(\der t)^i},
\end{equation*}
where we perform the standard Taylor expansion at the point $t=0$. Then, we only need the derives of $h^{i}(0)$, which can be estimated using only the score function. For instance, the $h^{(1)}(t)$ can be estimated with score estimations:
\begin{equation*}
    \begin{aligned}
        h^{(1)}(t) &= \grad f((\vz^\prime-\vz)\cdot t + \vz)\cdot (\vz^\prime - \vz)\\
        &\approx \tilde{h}^{(1)}(t) \coloneqq s_{\theta}((\vz^\prime-\vz)\cdot t + \vz) \cdot (\vz^\prime - \vz).
    \end{aligned}
\end{equation*}
Moreover, regarding the high-order derivatives, we can recursively perform the approximation: $\tilde{h}^{(i+1)}(0) = (\tilde{h}^{(i)}(\Delta t) - \tilde{h}^{(i)}(0))/\Delta t $.
Consider performing the approximation up to $u$-order derivatives, we can get the approximation of the energy difference:
\begin{equation*}
    r_{(K-k-1)\eta}(\vz^\prime, \vz) \coloneqq \sum_{i=1}^u\frac{\tilde{h}^{(i)}(0)}{i!}.
\end{equation*}
Then, the following corollary states the complexity of the score-only RTK-MALA algorithm.
\begin{corollary}
    Suppose the estimation errors of the score satisfies $\epsilon_{\mathrm{score}} \ll \rho\epsilon/(Ld^{1/2})$,
    and the log-likelihood function of $p_t$ has a bounded $u$-order derivative, e.g., $\left\|\grad^{(u)} f(\vz)\right\|\le L$,
    we have a non-parametric estimation for log-likelihood to make we have $\TVD{\hat{p}_{K\eta}}{p_*}\le \tilde{\mathcal{O}}(\epsilon)$ with a complexity shown as follows
    \begin{equation*}
        \tilde{\mathcal{O}}\left(L^4 \rho^{-3}\cdot \left(d+m_2^2\right)^2 Z^3\cdot \epsilon^{-2/(u-1)}\cdot 2^{u}\right).
    \end{equation*}
\end{corollary}
This result implies that if the energy function is infinite-order Lipschitz, we can nearly achieve any polynomial order convergence w.r.t. $\epsilon$ with the non-parametric energy difference estimation.


\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{cccc}
    \toprule
     Results & Algorithm & Assumptions &  Complexity \\
     \midrule
     \citet{chen2022sampling} & DDPM (SDE-based) & \ref{ass:lips_score},\ref{ass:second_moment},\ref{hat_e1} &  $\tilde{\mathcal{O}}(L^2d\epsilon^{-2})$\\
     \midrule
     \citet{chen2024probability} & DPOM (ODE-based) & \ref{ass:lips_score},\ref{ass:second_moment},\ref{hat_e1}, and $s_{\theta}$ smoothness &  $\tilde{\mathcal{O}}(L^3d\epsilon^{-2})$\\
     \midrule
     \citet{chen2024probability} & DPUM (ODE-based) & \ref{ass:lips_score},\ref{ass:second_moment},\ref{hat_e1}, and $s_{\theta}$ smoothness  &   $\tilde{\mathcal{\mathcal{O}}}(L^2d^{1/2}\epsilon^{-1})$\\
     \midrule
     \citet{li2023towards} &  ODE-based sampler & \ref{hat_e1} and estimation error of energy Hessian &   $\tilde{\mathcal{O}}(d^3\epsilon^{-1})$\\
     \midrule
     Corollary~\ref{cor:complexity_19_informal} & RTK-MALA & \ref{ass:lips_score},\ref{ass:second_moment},\ref{e1}, and \ref{e2} & \textcolor{red}{$\mathcal{O}(L^4 d^2 \log (d/\epsilon) )$}\\ 
     \midrule
     Theorem~\ref{thm:rtk_uld_complexity} & RTK-ULD (ours) & \ref{ass:lips_score},\ref{ass:second_moment},\ref{hat_e1} & \textcolor{red}{$\tilde{\mathcal{O}}(L^2d^{1/2}\epsilon^{-1})$}\\
     \bottomrule 
    \end{tabular}
    \caption{\small Comparison with prior works for RTK-based methods. The complexity denotes the number of calls for the score estimation to achieve $\TVD{\hat{p}_{K\eta}}{p_*}\le \tilde{\mathcal{O}}(\epsilon)$. $d$ and $\epsilon$ mean the dimension and error tolerance.
    Compared with the state-of-the-art result, RTK-ULD achieves the best dependence for both $d$ and $\epsilon$. Though RTK-MALA requires slightly stricter assumptions and worse dimension dependence, a linear convergence w.r.t. $\epsilon$ makes it suit high-accuracy sampling tasks.} 
    \label{tab:comp_old}
    %\vspace{-10pt}
\end{table*}

\begin{algorithm}[t]
    \caption{\sc ULD for RTK Inference}
    \label{alg:inner_uld}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:}  Returned particle of the previous iteration $\vx_0$, current iteration number $k$, inner iteration number $S$, inner step size $\tau$, velocity diffusion coefficient $\gamma$, required convergence accuracy $\epsilon$;
            \STATE Initialize the particle and velocity pair, i.e., $(\hat{\vz}_0, \hat{\vv}_0)$ with a Gaussian type product measure, i.e.,  $\mathcal{N}(\vzero, e^{2\eta}-1)\otimes \mathcal{N}(\vzero,\mI)$;
            \FOR{$t=s$ to $S-1$}
            \STATE Draw noise sample pair $(\xi^z_s,\xi^v_s)$ from a Gaussian type distribution.
            \STATE $\hat{\vz}_{s+1} = \hat{\vz}_{s} + \gamma^{-1} (1-e^{-\gamma \tau}) \hat{\vv}_{s} - \gamma^{-1} (\tau -\gamma^{-1} (1-e^{-\gamma \tau}) )s_\theta(\hat{\vz}_s) + \xi_s^z$
            \STATE $\hat{\vv}_{s+1} = e^{-\gamma\tau }\hat{\vv}_s - \gamma^{-1} (1-e^{-\gamma \tau}) 
 s_\theta(\hat{\vz}_s) + \xi^v_t$
            \ENDFOR
            \STATE {\bfseries return} $\vz_{S}$;
    \end{algorithmic}
\end{algorithm}

\paragraph{RTK-ULD.}
Alg.~\ref{alg:inner_uld} presents a solution employing ULD for the inner loop, which can accelerate the convergence of the inner loop due to the better discretization of the ULD algorithm. 
When it is used to solve the $k$-th sampling subproblem of Alg.~\ref{alg:rtk}, $\vx_0$ is equal to $\hat{\rvx}_{k\eta}$ defined in Section~\ref{sec:framework} and used to initialize particles iterating in Alg.~\ref{alg:inner_mala}.
Besides, the underlying distribution of noise sample pair is
{\small
\begin{equation*}
    \begin{aligned}
        (\xi^z_s,\xi^v_s)\sim &\mathcal{N}\left(\vzero,
            \left[
            \begin{matrix}
             \mM_{1,1} &  \mM_{1,2} \\
             \mM_{2,1} & \mM_{2,2}
            \end{matrix}
            \right]
        \right)\\
        \mathrm{where}\quad &\mM_{1,1} = \frac{2}{\gamma} \left( \tau - \frac{2}{\gamma} \left(1 - e^{-\gamma\tau} \right)\right) + \frac{1}{2\gamma} \left(1 - e^{-2\gamma\tau}\right)\mI\\
        &\mM_{1,2} = \mM_{2,1} = \frac{1}{\gamma} \left(1 - 2e^{-\gamma\tau} + e^{-2\gamma \tau}\right) \mI\\
        &\mM_{2,2} = \left(1-e^{-2\gamma\tau}\right)\cdot\mI
    \end{aligned}
\end{equation*}
}
In Alg.~\ref{alg:inner_uld}, we consider the process $\{(\hat{\rvz}_s, \hat{\rvv}_s)\}_{s=0}^S$ whose underlying distribution is denoted as $\{\hat{\pi}_s\}_{s=0}^{S}$.
We expect the $\vz$-marginal distribution of $\hat{\pi}_S$ to be close to the target distribution presented in Eq.~\ref{def:inner_target_dis}.
Unlike MALA, we only need to consider the error from score estimation in an expectation perspective, which is the same as that shown in~\cite{chen2022sampling}.
\begin{enumerate}[label=\textbf{[E{\arabic*}]}]
\setcounter{enumi}{2}
    \item \label{hat_e1}Estimation error of the score function: we assume a score estimator, e.g., a well-trained diffusion model, $s_{\theta}$, which can approximate the score function with an $\epsilon_{\mathrm{score}}$ error, i.e., $\E_{p_t}\left\|s_{\theta,t}(\vz) - \grad \log p_t(\vz)\right\|^2\leq \epsilon^2_{\mathrm{score}}$  for any $t\in[0,T]$.
\end{enumerate}
Under this condition, the complexity of RTK-ULD to achieve the convergence of TV distance is provided as follows, and the detailed proof is deferred to Theorem~\ref{thm:uld_outer_complexity_gene}.
Besides, we compare our theoretical results with the previous in Table~\ref{tab:comp_old}.
\begin{theorem}
    \label{thm:rtk_uld_complexity}
    Under Assumptions~\ref{ass:lips_score}--\ref{ass:second_moment} and \ref{hat_e1}, for Alg.~\ref{alg:rtk}, we choose 
    \begin{equation*}
        \begin{aligned}
             \eta= \frac{1}{2}\log \frac{2L+1}{2L},\quad K = 4L\cdot \log \frac{(1+L^2)d+\left\|\grad f_*(\vzero)\right\|^2}{\epsilon^2}
        \end{aligned}
    \end{equation*}
    and implement Step 3 of Alg.~\ref{alg:rtk} with projected Alg.~\ref{alg:inner_uld}.
    For the $k$-th run of Alg.~\ref{alg:inner_uld}, we require Gaussian-type initialization and high-accurate score estimation, i.e.,
    \begin{equation*}
        \hat{\pi}_0 = \mathcal{N}(\vzero, e^{2\eta}-1)\otimes \mathcal{N}(\vzero,\mI)\quad \mathrm{and}\quad \epsilon_{\mathrm{score}}=\tilde{\mathcal{O}}(\epsilon/\sqrt{L}).
    \end{equation*}
    If we set the hyperparameters of inner loops as follows. 
    the step size and the iteration number as
    \begin{equation*}
        \small
         \begin{aligned}
             \tau & = \tilde{\Theta}\left(\epsilon d^{-1/2} L^{-1/2} \cdot \left(\log \left[\frac{L(d+m_2^2+\|\vx_0\|^2)}{\epsilon^2}\right]\right)^{-1/2}\right)\\
            S &=\tilde{\Theta}\left(\epsilon^{-1}d^{1/2}\cdot \left(\log \left[\frac{L(d+m_2^2+\|\vx_0\|^2)}{\epsilon^2}\right]\right)^{1/2}\right).
         \end{aligned}
     \end{equation*}
    It can achieve $\TVD{\hat{p}_{K\eta}}{p_*}\lesssim \epsilon$
    with an $\tilde{\mathcal{O}}\left(L^2 d^{1/2}\epsilon^{-1} \right)$ gradient complexity.
\end{theorem}


\section{Conclusion and Limitation}

This paper presents an analysis of a modified version of diffusion models. Instead of focusing on the discretization of the reverse SDE,  we propose a general RTK framework that can produce a large class of algorithms for diffusion inference, which is formulated as solving a sequence of RTK sampling subproblems. Given this framework, we develop two algorithms called RTK-MALA and RTK-ULD, which leverage MALA and ULD to solve the RTK sampling subproblems. We develop theoretical guarantees for these two algorithms under certain conditions on the score estimation, and demonstrate their faster convergence rate than prior works. Numerical experiments support our theory.

We would also like to point out several limitations and future work. One potential limitation of this work is the lack of large-scale experiments. The main focus of this paper is the theoretical understanding and rigorous analysis of the diffusion process. Implementing large-scale experiments requires GPU resources and practitioner support, which can be an interesting direction for future work. Besides, though we provided a score-only RTK-MALA algorithm, the $\tilde{\mathcal{O}}(1/\epsilon)$ convergence rate can only be achieved by the RTK-MALA algorithm (Alg. \ref{alg:inner_mala}). However, this faster algorithm requires a direct approximation of the energy difference, which is not accessible in the existing pretrained diffusion model. Developing practical energy difference approximation algorithms and incorporating them with Alg. \ref{alg:inner_mala} for diffusion inference are also very interesting future directions.



==> 0_contents/backup.tex <==

including its implementation by the Markov process $\{\hat{\rvx}_{k\eta}\}$, and some fundamental properties.
The key idea of this framework is to divide the entire generation process into a series of sampling subproblems whose target distribution is the RTK of the forward process, i.e., $p_{(K-k-1)\eta|(K-k)\eta}$ for the $k$-th transition.
Since the forward process is an OU process, the closed form of RTK, i.e., $p_{t|t^\prime}$, can be calculated explicitly for any $t^\prime\ge t$.
Then, combining the smoothness properties of $p_t$, we find that RTK can be formulated to be a strongly log-concave distribution when $\eta$ is chosen as a constant level.
Moreover, strongly log-concave target distributions for the $k$-th transition can be approximated by $\hat{p}_{(k+1)\eta|k\eta}$ through any posterior sampling algorithm.
As a result, we can consider the entire generation process to be $K$ sampling subproblems where $K=\tilde{\mathcal{O}}(1)$.

Different from the paradigm of DDPM, we construct a Markov process, i.e., $\{\hat{\rvx}_k\}$, with underlying distributions $\hat{p}_{k\eta}$.
This process initializes $\hat{\rvx}_0$ with the standard Gaussian and then approximates the strongly log-concave target distributions of the sampling subproblem $p_{(K-k-1)\eta|(K-k)\eta}(\cdot|\vx)$, by $\hat{p}_{(k+1)\eta|k\eta}(\cdot|\vx)$ with high accuracy in TV or KL metrics.

\begin{figure}[t]
    \centering
    \input{0_figures/rds_illu_step_1}
    \caption{\small The illustration of the three Markov processes, i.e., $\left\{\rvx_t\right\}$, $\left\{\rbkwx_t\right\}$ and $\left\{\hat{\rvx}_t\right\}$, in Section~\ref{sec:pre}. The top of the figure describes the underlying distribution of $\{\rvx_t\}$, i.e.,  SDE.~\ref{sde:ou}, and the middle presents the process $\{\rbkwx_t\}$, SDE.~\ref{def:rev_ou_sde_prac}.
    For the bottom part, the line denotes the process $\{\hat{\rvx}_t\}$ introducing a log-concave transition kernel to approximate $p_{T-(k+1)\eta|T-k\eta}$ with $\hat{p}_{(k+1)\eta|k\eta}$ which satisfies ~\ref{ineq:tvd_appro} or~\ref{ineq:kld_appro}. }
    \label{con_fig:rrds_forward}
\end{figure}

\subsection{Discussion}

Note that both MALA and ULD inner-loop can obtain a good convergence rate, the key point is that our implementation of RTK allows larger learning rate so that the convergence can be faster than reverse SDE discretization. This idea can also be implemented with any other MCMC algorithm as the inner loop solver. From the technical side, the error analysis of the inner loop elucidate the total complexity of the algorithm and the dependency on the inner error and score/energy function estimation error.

==> 0_figures/rds_illu_backup.tex <==
\usetikzlibrary{decorations.pathreplacing}

\begin{tikzpicture}

%\node at (5,4.9) {The forward process};

%\node at (5,-1) {The reverse process};

\filldraw (0,4) circle (0.05); \node at (-0.2, 3.7) {\textcolor{red}{$p_{0}=p_*$}}; 
\draw[-latex]  (0,4)--(0.5,4);
\draw[densely dotted] (0.5,4)--(1.5,4);
\draw[-latex]  (1.5,4)--(2,4);
\filldraw (2,4) circle (0.05); \node at (1.8, 3.7) {$p_{T-(k+1)\eta}$}; 
\filldraw (5,4) circle (0.05); \node at (4.8, 3.7) {$p_{T-k\eta-\tau}$};
\draw[-] (2,4)--(5,4);
\draw[-] (5,4)--(8,4);
\filldraw (8,4) circle (0.05); \node at (7.8, 3.7) {$p_{T-k\eta}$}; 
\draw[-latex]  (8,4)--(8.5,4);
\draw[densely dotted] (8.5,4)--(9.5,4);
\draw[-latex]  (9.5,4)--(10,4);
\filldraw (10,4) circle (0.05); \node at (9.8, 3.7) {\textcolor{blue}{$p_{T}\quad\approx$}}; 
\draw[dashed] (10,4)--(11, 4);
\filldraw (11,4) circle (0.05); \node at (11.2, 3.7) {$p_\infty$}; 

\filldraw (0,0) circle (0.05); \node at (-0.2, -0.3) {\textcolor{red}{$\bkwp_{T}$}}; 
\draw[-latex]  (0.5,0)--(0,0);
\draw[densely dotted] (0.5,0)--(1.5,0);
\draw[-latex]  (2,0)--(1.5,0);
\filldraw (2,0) circle (0.05); \node at (1.8, -0.3) {$\bkwp_{(k+1)\eta}$}; 
\filldraw (5,0) circle (0.05); \node at (4.8, -0.3) {$\bkwp_{k\eta +\tau}$}; 
\draw[-] (2,0)--(5,0);
\draw[-] (5,0)--(8,0);
\filldraw (8,0) circle (0.05); \node at (7.8, -0.3) {$\bkwp_{k\eta}$}; 
\draw[-latex]  (8.5,0)--(8,0);
\draw[densely dotted] (8.5,0)--(9.5,0);
\draw[-latex]  (10,0)--(9.5,0);
\filldraw (10,0) circle (0.05); \node at (9.8, -0.3) {\textcolor{blue}{$\bkwp_{0}$}}; 


\draw[dashed] (0,0)--(0,4);
\draw[dashed] (10,0)--(10,4);
\node [rotate=90] at (-0.3,2) {$\approx$};
\draw[-] (11,4)--(10,0);
\node [rotate=72] at (10.8,2) {$=$};

\filldraw (2,1) circle (0.05); \node at (1.8, 1.3) {$\rbkwv_{k+1}$}; 
\filldraw (8,1) circle (0.05); \node at (8.3, 1.3) {$\rbkwv_{k}$}; 
\filldraw (5,1) circle (0.05); \node at (5.3, 1.3) {$\rbkwv_{k}$}; 
\draw[-latex, dashed] (2,0)--(2,1);
\draw[-latex, dashed] (8,0)--(8,1);
\draw[-latex, dashed] (5,0)--(5,1);






\filldraw (2,3) circle (0.05); \node at (1.8, 2.7) {$\grad\ln p_{T-(k+1)\eta}$}; 
\filldraw (8,3) circle (0.05); \node at (8.3, 2.7) {$\grad\ln p_{T-k\eta}$}; 
\draw[-latex, dashed] (2,4)--(2,3);
\draw[-latex, dashed] (8,4)--(8,3);
\filldraw (5,3) circle (0.05); \node at (5.3, 2.7) {$\grad\ln p_{T-k\eta-\tau}$}; 
\draw[-latex, dashed] (5,4)--(5,3);




\end{tikzpicture}

==> 0_figures/rds_illu_step_1.tex <==
\usetikzlibrary{decorations.pathreplacing}

\begin{tikzpicture}

%\node at (5,4.9) {The forward process};

%\node at (5,-1) {The reverse process};

\filldraw (0,3.6) circle (0.05); \node at (-0.2, 3.3) {\textcolor{red}{$p_{0}=p_*$}}; 
\draw[-latex]  (0,3.6)--(0.5,3.6);
\draw[densely dotted] (0.5,3.6)--(1.5,3.6);
\draw[-latex]  (1.5,3.6)--(2,3.6);
\filldraw (2,3.6) circle (0.05); \node at (1.8, 3.3) {$p_{T-(k+1)\eta}$}; 
\draw[-] (2,3.6)--(5,3.6);
\draw[-] (5,3.6)--(8,3.6);
\filldraw (8,3.6) circle (0.05); \node at (7.8, 3.3) {$p_{T-k\eta}$}; 
\draw[-latex]  (8,3.6)--(8.5,3.6);
\draw[densely dotted] (8.5,3.6)--(9.5,3.6);
\draw[-latex]  (9.5,3.6)--(10,3.6);
\filldraw (10,3.6) circle (0.05); \node at (9.8, 3.3) {\textcolor{blue}{$p_{T}\quad\approx$}}; 
\draw[dashed] (10,3.6)--(11, 3.6);
\filldraw (11,3.6) circle (0.05); \node at (11.2, 3.3) {$p_\infty$}; 

\filldraw (0,0) circle (0.05); \node at (-0.2, -0.3) {\textcolor{red}{$\bkwp_{T}$}}; 
\draw[-latex]  (0.5,0)--(0,0);
\draw[densely dotted] (0.5,0)--(1.5,0);
\draw[-latex]  (2,0)--(1.5,0);
\filldraw (2,0) circle (0.05); \node at (1.8, -0.3) {$\bkwp_{(k+1)\eta}$}; 
\draw[-] (2,0)--(5,0);
\draw[-] (5,0)--(8,0);
\filldraw (8,0) circle (0.05); \node at (7.8, -0.3) {$\bkwp_{k\eta}$}; 
\draw[-latex]  (8.5,0)--(8,0);
\draw[densely dotted] (8.5,0)--(9.5,0);
\draw[-latex]  (10,0)--(9.5,0);
\filldraw (10,0) circle (0.05); \node at (9.8, -0.3) {\textcolor{blue}{$\bkwp_{0}$}}; 


\draw[dashed] (0,0)--(0,3.6);
\draw[dashed] (10,0)--(10,3.6);
\node [rotate=90] at (-0.3,2) {$\approx$};
\draw[-] (11,3.6)--(10,0);
\node [rotate=72] at (10.8,2) {$=$};

\filldraw (2,1) circle (0.05); \node at (1.8, 1.3) {$\vs_{\theta,(k+1)\eta}$}; 
\node at (5, 1.3) {A \textbf{Gaussian} transition}; 
\node at (5, 0.8) {$\bkwp_{(k+1)\eta|k\eta}$};
\draw[-latex] (8,0)..controls (7.5,0.5)and(6.5,0.7)..(6, 0.8);
\draw[-latex] (4,0.8)..controls (3.5,0.7)and(2.5,0.5)..(2, 0);
\filldraw (8,1) circle (0.05); \node at (8.3, 1.3) {$\vs_{\theta, k\eta}$}; 
\draw[-latex, dashed] (2,0)--(2,1);
\draw[-latex, dashed] (8,0)--(8,1);






\filldraw (2,2.6) circle (0.05); \node at (1.8, 2.3) {$\grad\ln p_{T-(k+1)\eta}$}; 
\node at (5, 2.3) {The reverse transition};
\node at (5, 2.8) {$p_{T-(k+1)\eta|T-k\eta}$};
\draw[-latex] (8,3.6)..controls (7.5,3.1)and(6.5,2.9)..(6.3, 2.8);
\draw[-latex] (3.7,2.8)..controls (3.5,2.9)and(2.5,3.1)..(2, 3.6);
\filldraw (8,2.6) circle (0.05); \node at (8.3, 2.3) {$\grad\ln p_{T-k\eta}$}; 
\draw[-latex, dashed] (2,3.6)--(2,2.6);
\draw[-latex, dashed] (8,3.6)--(8,2.6);


\filldraw (0,-2.4) circle (0.05); \node at (-0.2, -2.7) {\textcolor{red}{$\hat{p}_{T}$}}; 
\draw[-latex]  (0.5,-2.4)--(0,-2.4);
\draw[densely dotted] (0.5,-2.4)--(1.5,-2.4);
\draw[-latex]  (2,-2.4)--(1.5,-2.4);
\filldraw (2,-2.4) circle (0.05); \node at (1.8, -2.7) {$\hat{p}_{(k+1)\eta}$}; 
\draw[-] (2,-2.4)--(5,-2.4);
\draw[-] (5,-2.4)--(8,-2.4);
\filldraw (8,-2.4) circle (0.05); \node at (7.8, -2.7) {$\hat{p}_{k\eta}$}; 
\draw[-latex]  (8.5,-2.4)--(8,-2.4);
\draw[densely dotted] (8.5,-2.4)--(9.5,-2.4);
\draw[-latex]  (10,-2.4)--(9.5,-2.4);
\filldraw (10,-2.4) circle (0.05); \node at (9.8, -2.7) {\textcolor{blue}{$\hat{p}_{0}$}}; 

\filldraw (2,-1.4) circle (0.05); \node at (1.8, -1.1) {$\vs_{\theta,(k+1)\eta}$}; 
\node at (5, -1.1) {A \textbf{log-concave} transition}; 
\node at (5, -1.6) {$\hat{p}_{(k+1)\eta|k\eta}$};
\draw[-latex] (8,-2.4)..controls (7.5,-1.9)and(6.5,-1.7)..(6, -1.6);
\draw[-latex] (4,-1.6)..controls (3.5,-1.7)and(2.5,-1.9)..(2, -2.4);
\filldraw (8,-1.4) circle (0.05); \node at (8.3, -1.1) {$\vs_{\theta, k\eta}$}; 
\draw[-latex, dashed] (2,-2.4)--(2,-1.4);
\draw[-latex, dashed] (8,-2.4)--(8,-1.4);


\draw[-latex, dashed] (0,-2.4)--(0,0);
\draw[-latex, dashed] (10,-2.4)--(10,0);
\node [rotate=90] at (-0.3,-1.4) {$\approx$};


\draw[-] (11,3.6)--(10,-2.4);
\node [rotate=80] at (10.8,-0.2) {$=$};

\end{tikzpicture}
